Temperature dependence of quantum oscillations from non-parabolic dispersions

The phase offset of quantum oscillations is commonly used to experimentally diagnose topologically non-trivial Fermi surfaces. This methodology, however, is inconclusive for spin-orbit-coupled metals where $\pi$-phase-shifts can also arise from non-topological origins. Here, we show that the linear dispersion in topological metals leads to a $T^2$-temperature correction to the oscillation frequency that is absent for parabolic dispersions. We confirm this effect experimentally in the Dirac semi-metal Cd$_3$As$_2$ and the multiband Dirac metal LaRhIn$_5$. Both materials match a tuning-parameter-free theoretical prediction, emphasizing their unified origin. For topologically trivial Bi$_2$O$_2$Se, no frequency shift associated to linear bands is observed as expected. However, the $\pi$-phase shift in Bi$_2$O$_2$Se would lead to a false positive in a Landau-fan plot analysis. Our frequency-focused methodology does not require any input from ab-initio calculations, and hence is promising for identifying correlated topological materials.

==> preamble.tex <==
%\pdfoutput=1
\setlength{\intextsep}{10pt}
\setlength{\textfloatsep}{5pt}

%adjust height of rows in a table
\setlength\extrarowheight{2.5pt}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

%% ultimate commands
	
	% align environment
			\newcommand{\e}[1]{\begin{align}{#1}\end{align}}	
	
		
	% fraction
		\newcommand{\f}[2]{\frac{#1}{#2}}
		\newcommand{\tf}[2]{\tfrac{#1}{#2}}
		
	% partial differentiation
		\newcommand{\p}[2]{\frac{\partial #1}{\partial #2}}
		\newcommand{\pf}[3]{\frac{\partial #1}{\partial #2}\bigg|_{#3}}
		\newcommand{\pa}[1]{\partial_{#1}}
		
	% label equations/sections
		\newcommand{\la}[1]{\label{#1}}

	% refer to equation, section, figure, appendix
		\newcommand{\q}[1]{Eq.\ (\ref{#1})}
		\newcommand{\qq}[2]{Eqs.\ (\ref{#1})-(\ref{#2})}
		\newcommand{\s}[1]{Sec.\ \ref{#1}}
		\newcommand{\fig}[1]{Fig.\ \ref{#1}}		
		\newcommand{\app}[1]{App.\ \ref{#1}}				
		\newcommand{\tab}[1]{Tab.\ \ref{#1}}
		\newcommand{\ocite}[1]{Ref.\ \onlinecite{#1}}
		\newcommand{\cf}[1]{[cf.\ Eq.\ (\ref{#1})]}
	
				
	% brackets
		\newcommand{\brac}[1]{\left(\;#1\;\right)}
		\newcommand{\sq}[1]{\left[\;#1\;\right]}
		\newcommand{\cu}[1]{\left\{\;#1\;\right\}}

	% insert words in equation environment

		\newcommand{\iwith}{\ins{with}}
		\newcommand{\where}{\ins{where}}		
		\newcommand{\iand}{\ins{and}}
		\newcommand{\ior}{\ins{or}}
		\newcommand{\ifor}{\ins{for}}
		\newcommand{\st}{\ins{s.t.}}
		
	% sign functions
		\newcommand{\sgn}{\text{sgn}}

	% equal, approximate, proportional signs, limits
		\newcommand{\eq}{=&\;}
		\newcommand{\condeq}[1]{\as \substack{\sma{#1}\\=}\as}
		\newcommand{\condprop}[1]{\as \substack{\sma{#1}\\ \propto}\as}
		\newcommand{\limit}[1]{\substack{\text{lim}\\#1}\as}		
		\newcommand{\appr}{\approx &\;}
		\newcommand{\prop}{\propto&\;}
		\newcommand{\define}{\as\substack{\text{def}\\ \iff}\as}					
	
	% mathbb symbols
		\newcommand{\F}{\mathbb{F}}
		\newcommand{\R}{\mathbb{R}}
		\newcommand{\Z}{\mathbb{Z}}
		\newcommand{\I}{\mathbb{I}}
		\newcommand{\C}{\mathbb{C}}
		\newcommand{\N}{\mathbb{N}}		
		\newcommand{\Q}{\mathbb{Q}}				
		\newcommand{\bbs}{\mathbb{S}}
		\newcommand{\bbt}{\mathbb{T}}

		
% for review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

% exponential 
\newcommand{\ex}{\text{exp}}
\newcommand{\pexp}{\overline{\text{exp}}}
		
		
% plane wave
	\newcommand{\eikr}{e^{i\bk \cdot \br}}
	\newcommand{\eikR}{e^{i\bk \cdot \bR}}
	\newcommand{\emikr}{e^{-i\bk \cdot \br}}
	\newcommand{\emikR}{e^{-i\bk \cdot \bR}}	

% divergence,curl,laplacian
\newcommand{\na}{\nabla}
\newcommand{\nai}{\nabla_i}
\newcommand{\naj}{\nabla_j}
\newcommand{\nak}{\nabla_k}
\newcommand{\nal}{\nabla_l}
\newcommand{\diverge}{\nabla \cdot}
\newcommand{\curl}{\nabla \times}
\newcommand{\lap}{\nabla^2}
\newcommand{\nabr}{\nabla_{\boldsymbol{r}}}
\newcommand{\nabk}{\nabla_{\boldsymbol{k}}}
\newcommand{\nabkp}{\nabla_{\boldsymbol{k}'}}

%fundamental constants
\newcommand{\bohr}{\mu_{\sma{B}}}
\newcommand{\gfac}{g_{\sma{0}}}
\newcommand{\lmt}{l^{\mt}}
\newcommand{\lmf}{l^{\text{-}4}}
\newcommand{\lmo}{l^{\mo}}




% specific to geometric_orbital
\newcommand{\om}{orbital moment }
\newcommand{\omm}{orbital moment}
\newcommand{\zf}{Zilberman-Fischbeck }
\newcommand{\checkgp}{\check{g}^{\sma{\perp}}}
\newcommand{\btperp}{$BT_{\sma{\perp}}$}
\newcommand{\bise}{Bi$_2$Se$_3$}



% c creation operators

\newcommand{\cdagk}{\dg{c}_{\bk}}
\newcommand{\ck}{\pdg{c}_{\bk}}
\newcommand{\cdagksig}{\dg{c}_{\bk,\sigma}}
\newcommand{\cksig}{\pdg{c}_{\bk,\sigma}}
\newcommand{\cdagkup}{c^\dagger_{\boldsymbol{k}\uparrow}}
\newcommand{\cdagkdo}{c^\dagger_{\boldsymbol{k}\downarrow}}
\newcommand{\ckup}{\pdg{c}_{\boldsymbol{k} \uparrow}}
\newcommand{\ckdo}{\pdg{c}_{\boldsymbol{k} \downarrow}}

\newcommand{\cdag}[1]{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{#1}}}
\newcommand{\cnod}[1]{c_{\scriptstyle{#1}}}


\newcommand{\cdj}{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{j \sigma}}}
\newcommand{\cnj}{c_{\scriptstyle{j' \sigma'}}}


% f creation operator

\newcommand{\fsig}{\pdg{f}_{\sigma}}
\newcommand{\fdagsig}{\dg{f}_{\sigma}}
\newcommand{\fup}{\pdg{f}_{\uparrow}}
\newcommand{\fdagup}{\dg{f}_{\uparrow}}
\newcommand{\fdo}{\pdg{f}_{\downarrow}}
\newcommand{\fdagdo}{\dg{f}_{\downarrow}}


%levi Cevita
\newcommand{\levi}[1]{\epsilon_{#1}}


%spin symbols
\newcommand\nup{\hat{n}_{f\uparrow}}
\newcommand\ndo{\hat{n}_{f\downarrow}}
\newcommand\avenup{{n}_{f\uparrow}}
\newcommand\avendo{{n}_{f\downarrow} }

% energies with varepsilon
\newcommand{\var}{\varepsilon}
%\newcommand{\var}[1]{\varepsilon_{#1}}
\newcommand{\efu}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\uparrow}}}
\newcommand{\efd}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\downarrow}}}
\newcommand{\ef}{\varepsilon_{\scriptscriptstyle{f}}}
\newcommand{\EF}{E_{\scriptscriptstyle{F}}}
\newcommand{\ek}{\varepsilon_{\boldsymbol{k}}}
\newcommand{\eF}{\varepsilon_{\scriptscriptstyle{F}}}
\newcommand{\enk}{\varepsilon_{n,\bk}}




% space

\newcommand\as{\;\;\;\;}
\newcommand\ass{\;\;\;\;\;\;\;\;}


\newcommand\Wline[2]{ \pdg{\W}_{\sma{#1 \leftarrow #2}}}


%hat operators

\newcommand{\hn}{\hat{n}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hO}{\hat{O}}
\newcommand{\hPi}{\hat{{\Pi}}}
\newcommand{\hpsi}{\hat{{\psi}}}
\newcommand{\hphi}{\hat{{\phi}}}
\newcommand{\hrho}{\hat{{\rho}}}
\newcommand{\hsigma}{\hat{{\sigma}}}
	%hatted operators with dagger
	\newcommand{\dhpsi}{\dg{\hat{{\psi}}}}
	\newcommand{\dhphi}{\dg{\hat{{\phi}}}}


%hatted bold symbols
\newcommand{\hbp}{\hat{\bp}}
\newcommand{\hbr}{\hat{\br}}
\newcommand{\hbv}{\hat{\bv}}
\newcommand{\hbx}{\hat{\bx}}
\newcommand{\bhp}{\boldsymbol{\hat{p}}}
\newcommand{\hbA}{\hat{\bA}}
\newcommand{\hbB}{\hat{\bB}}
\newcommand{\hbJ}{\hat{\bJ}}
\newcommand{\hbP}{\hat{\bP}}
\newcommand{\hbpi}{\hat{\boldsymbol{\pi}}}
\newcommand{\hbPi}{\hat{\boldsymbol{\Pi}}}


%bold symbols

\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bkp}{\boldsymbol{k}_{\sma{\perp}}}
\newcommand{\bkpar}{\bk_{\parallel}}
\newcommand{\bkone}{\boldsymbol{k_1}}
\newcommand{\bktwo}{\boldsymbol{k_2}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\brp}{\boldsymbol{r}_{\sma{\perp}}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bze}{\boldsymbol{0}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bcalf}{\boldsymbol{\calf}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarpi}{\boldsymbol{\varpi}}
\newcommand{\bdeltapar}{\boldsymbol{\delta}_{\sma{\parallel}}}
\newcommand{\bna}{\boldsymbol{\nabla}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}



%\mathfrak
\newcommand{\frake}{\mathfrak{e}}
\newcommand{\frako}{\mathfrak{o}}
\newcommand{\frakt}{\mathfrak{t}}
\newcommand{\fraks}{\mathfrak{s}}
\newcommand{\frakr}{\mathfrak{r}}
\newcommand{\mx}{\mathfrak{X}}
\newcommand{\mxx}{\mathfrak{X}^x}
\newcommand{\mxy}{\mathfrak{X}^y}
\newcommand{\bmx}{\bar{M}_x}


\newcommand{\orb}{\boldsymbol{\mathfrak{A}}}
\newcommand{\lutt}{\boldsymbol{\mathfrak{L}}}



%tilde
\newcommand{\tbPi}{\tilde{\bPi}}
\newcommand{\tPi}{\tilde{\Pi}}
\newcommand{\txi}{\tilde{\xi}}
\newcommand{\tbv}{\tilde{\bv}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tbmx}{\tilde{\bmx}}
\newcommand{\tmxx}{\tilde{\mx}^x}
\newcommand{\tmxy}{\tilde{\mx}^y}
\newcommand{\tmx}{\tilde{\mx}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tbsigma}{\tilde{\bsigma}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\tilu}[1]{\tilde{u}_{#1}}
\newcommand\tilX{\tilde{X}}
\newcommand\tilZ{\tilde{Z}}
\newcommand\tilGamma{\tilde{\Gamma}}
\newcommand\tilU{\tilde{U}}

%calligraphic
\newcommand{\calL}{{\cal L}}
\newcommand{\W}{{\cal W}}
\newcommand{\A}{{\cal A}}


% equal signs
\newcommand\kzeq{\;\stackrel{\mathclap{\normalfont\mbox{$\sma{\bar{k}_z}$}}}{=}\;}

%breve 
\newcommand{\breveg}{\breve{g}}


% symmetry operators
\newcommand{\inv}{\mathfrak{i}}
\newcommand{\mir}{\mathfrak{r}}
\newcommand\glide{\mathfrak{g}}
\newcommand\rot{\mathfrak{c}}
\newcommand\scr{\mathfrak{s}}
\newcommand\tra{\mathfrak{t}}


\newcommand{\calti}{{\cal T}_{\sma{\cal I}}}
\newcommand{\gdel}{g_{\boldsymbol{\delta}}}
\newcommand{\pgdel}{\pdg{g}_{\boldsymbol{\delta}}}
\newcommand{\bmz}{\bar{M}_z}
\newcommand{\calbmx}{{\cal \bar{M}}_x}
\newcommand{\calgdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevegdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevebmx}{\breve{\bar{M}}_x}
\newcommand{\uit}{U_{\sma{\cali T}}}
\newcommand{\utg}{U_{\sma{Tg \bdelta}}}
\newcommand{\ut}{U_{\sma{T}}}
\newcommand{\ug}{U_{\sma{g \bdelta}}}
\newcommand{\ubmx}{U_{\sma{\bmx}}}
\newcommand{\utbmz}{U_{\sma{T\bmz}}}
\newcommand{\calug}{\calg_{\sma{\bdelta}}}
\newcommand{\caluit}{\calu_{\sma{\cali T}}}
\newcommand{\caltgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetbmx}{\breve{T}_{\sma{\bmx}}}
\newcommand{\hattbmx}{\hat{T}_{\sma{\bmx}}}
\newcommand{\brevetbmz}{\breve{T}_{\sma{\bmz}}}
\newcommand{\breveti}{\breve{T}_{\sma{\cali}}}
\newcommand{\caltbmz}{\calt_{\sma{\bmz}}}
\newcommand{\caltbmx}{\calt_{\sma{\bmx}}}
\newcommand{\calut}{\calu_{\sma{T}}}
\newcommand{\hatgdel}{\pdg{\hat{g}}_{\sma{\bdelta}}}
\newcommand{\hatTg}{\pdg{\hat{T}}_{\sma{g\bdelta}}}
\newcommand\csixdel{C_{\sma{6,\bdelta}}}
\newcommand\brevecsixdel{\breve{C}_{\sma{6,\bdelta}}}
\newcommand\cthreedel{C_{\sma{3,\bdelta}}}
\newcommand\brevecthreedel{\breve{C}_{\sma{3,\bdelta}}}
\newcommand\hatcthreedel{\hat{C}_{\sma{3,\bdelta}}}
\newcommand\cthreetwodel{C_{\sma{3,2\bdelta}}}
\newcommand\brevecthreetwodel{\breve{C}_{\sma{3,2\bdelta}}}
\newcommand\brevectwothreedel{\breve{C}_{\sma{2,3\bdelta}}}
\newcommand\ctwothreedel{C_{\sma{2,3\bdelta}}}
\newcommand\hatcsixdel{\hat{C}_{\sma{6,\bdelta}}}
\newcommand\ucsixdel{U_{\sma{C_6,\bdelta}}}
\newcommand\cndel{C_{\sma{n,\bdelta}}}
\newcommand\cbarndel{C_{\sma{\bar{n},\bdelta}}}
\newcommand\ucndel{U_{\sma{C_n,\bdelta}}}
\newcommand\hatcndel{\hat{C}_{\sma{n,\bdelta}}}
\newcommand\brevecndel{\breve{C}_{\sma{n,\bdelta}}}
\newcommand\brevectwotwodel{\breve{C}_{\sma{2,2\bdelta}}}
\newcommand\brevecfourdel{\breve{C}_{\sma{4,\bdelta}}}
\newcommand\brevectwodel{\breve{C}_{\sma{2,\bdelta}}}


% vectors and matrices
\newcommand{\vectwo}[2]{\begin{pmatrix} {#1}\\{#2} \end{pmatrix}}
\newcommand{\matrixtwo}[4]{\begin{pmatrix} #1 & #2 \\ #3 & #4 \end{pmatrix}}
\newcommand{\diagmatrix}[2]{\begin{pmatrix} #1 & 0 \\ 0 & #2 \end{pmatrix}}
\newcommand{\matrixthree}[9]{\begin{pmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{pmatrix}}


% Pauli matrices
\newcommand{\szero}{\sigma_{\sma{0}}}
\newcommand{\sx}{\sigma_{\sma{1}}}
\newcommand{\sy}{\sigma_{\sma{2}}}
\newcommand{\sz}{\sigma_{\sma{3}}}
\newcommand{\tzero}{\tau_{\sma{0}}}
\newcommand{\tx}{\tau_{\sma{1}}}
\newcommand{\ty}{\tau_{\sma{2}}}
\newcommand{\tz}{\tau_{\sma{3}}}



% parafermion operators
\newcommand{\gt}{\gamma_{\sma{2}}}
\newcommand{\gth}{\gamma_{\sma{3}}}
\newcommand{\gfo}{\gamma_{\sma{4}}}
\newcommand{\gfi}{\gamma_{\sma{5}}}
\newcommand{\gj}{\gamma_{\sma{j}}}
\newcommand{\gtj}{\gamma_{\sma{2j}}}
\newcommand{\gtjpo}{\gamma_{\sma{2j+1}}}
\newcommand{\gtjpt}{\gamma_{\sma{2j+2}}}
\newcommand{\gtjmo}{\gamma_{\sma{2j-1}}}
\newcommand{\gtL}{\gamma_{\sma{2L}}}
\newcommand{\gtLpo}{\gamma_{\sma{2L+1}}}
\newcommand{\gtLpt}{\gamma_{\sma{2L+2}}}
\newcommand{\gtLmo}{\gamma_{\sma{2L-1}}}
\newcommand{\gtLmt}{\gamma_{\sma{2L-2}}}
\newcommand{\gtLmth}{\gamma_{\sma{2L-3}}}
\newcommand{\gtLmfo}{\gamma_{\sma{2L-4}}}


% insert text in equation
\newcommand{\ins}[1]{\;\;\;\;\text{#1}\;\;\;\;}


%momentum parallel and perpendicular
\newcommand{\kpar}{\boldsymbol{k}_{{\shortparallel}}}
\newcommand{\Dpar}{D^{g}_{{\shortparallel}}}
\newcommand{\kper}{k_{\perp}}


% Cnv 
\newcommand{\ctv}{C_{3v}}
\newcommand{\cfv}{C_{4v}}
\newcommand{\csv}{C_{6v}}
\newcommand{\cnv}{C_{nv}}


%C_n Time-reversal
\newcommand{\cnt}{C_n {\cal T}}
\newcommand{\cn}{C_n}
\newcommand{\cfour}{C_4}
\newcommand{\cs}{C_6}
\newcommand{\ct}{C_3}
\newcommand{\cst}{C_6{\cal T}}
\newcommand{\cft}{C_4{\cal T}}
\newcommand{\ctt}{C_2{\cal T}}


% average 
\newcommand{\ave}[1]{\langle\,#1\,\rangle}



%inverse Angstroms and Angstroms
\newcommand{\invA}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}
\newcommand{\ang}{\mathrm{\AA}}

% Lagrangian
\newcommand{\lag}{{\mathscr{L}}}


% green's function
\newcommand{\green}{{\mathscr{G}}}

% Cauchy principal value
\newcommand{\prin}{{\mathscr{P}}}

% imaginary and real parts
\newcommand{\imag}{{\mathscr{I}}}
\newcommand{\real}{{\mathscr{R}}}


%total differentiation
\newcommand{\totaldif}[2]{\frac{ d #1}{d #2}}

% calligraphic font
\newcommand{\cala}{{\cal A}}
\newcommand{\calb}{{\cal B}}
\newcommand{\calc}{{\cal C}}
\newcommand{\cald}{{\cal D}}
\newcommand{\cale}{{\cal E}}
\newcommand{\calf}{{\cal F}}
\newcommand{\calg}{{\cal G}}
\newcommand{\calh}{{\cal H}}
\newcommand{\tcalh}{\tilde{\cal H}}
\newcommand{\cali}{{\cal I}}
\newcommand{\calj}{{\cal J}}
\newcommand{\calk}{{\cal K}}
\newcommand{\call}{{\cal L}}
\newcommand{\calm}{{\cal M}}
\newcommand{\caln}{{\cal N}}
\newcommand{\calo}{{\cal O}}
\newcommand{\calp}{{\cal P}}
\newcommand{\calq}{{\cal Q}}
\newcommand{\calr}{{\cal R}}
\newcommand{\cals}{{\cal S}}
\newcommand{\calt}{{\cal T}}
\newcommand{\calu}{{\cal U}}
\newcommand{\calv}{{\cal V}}
\newcommand{\calw}{{\cal W}}
\newcommand{\calx}{{\cal X}}
\newcommand{\caly}{{\cal Y}}
\newcommand{\calz}{{\cal Z}}

% mathscript font
\newcommand{\scra}{{\mathscr A}}
\newcommand{\scrb}{{\mathscr B}}
\newcommand{\scrc}{{\mathscr C}}
\newcommand{\scrd}{{\mathscr D}}
\newcommand{\scre}{{\mathscr E}}
\newcommand{\barscre}{\bar{\mathscr E}}
\newcommand{\scrf}{{\mathscr F}}
\newcommand{\scrg}{{\mathscr G}}
\newcommand{\scrh}{{\mathscr H}}
\newcommand{\tscrh}{\tilde{\mathscr H}}
\newcommand{\scri}{{\mathscr I}}
\newcommand{\scrj}{{\mathscr J}}
\newcommand{\scrk}{{\mathscr K}}
\newcommand{\scrl}{{\mathscr L}}
\newcommand{\scrm}{{\mathscr M}}
\newcommand{\scrn}{{\mathscr N}}
\newcommand{\scro}{{\mathscr O}}
\newcommand{\scrp}{{\mathscr P}}
\newcommand{\scrq}{{\mathscr Q}}
\newcommand{\scrr}{{\mathscr R}}
\newcommand{\scrs}{{\mathscr S}}
\newcommand{\scrt}{{\mathscr T}}
\newcommand{\scru}{{\mathscr U}}
\newcommand{\scrv}{{\mathscr V}}
\newcommand{\scrw}{{\mathscr W}}
\newcommand{\scrx}{{\mathscr X}}
\newcommand{\scry}{{\mathscr Y}}
\newcommand{\scrz}{{\mathscr Z}}


%Gamma matrices
\newcommand{\gam}[1]{\Gamma_{#1}}

%determinant
\newcommand{\de}[1]{\text{det}[\;#1\;]}

%trace
\newcommand{\tr}{\text{Tr}}




\newcommand{\noi}[1]{\noindent (#1)}
\newcommand{\imp}{\;\;\Rightarrow\;\;}
\newcommand{\mo}{\text{-}1}
\newcommand{\mt}{\text{-}2}
\newcommand{\minus}{\text{-}}
\newcommand{\oneover}[1]{\tfrac{1}{#1}}


% A command for inner product and bras and kets
\newcommand{\braket}[2]{\big\langle #1 \big| #2 \big\rangle}
\newcommand{\ketbra}[2]{\big|  #1  \big\rangle \big\langle #2 \big| }
\newcommand{\braopket}[3]{\big\langle #1 \big| #2 \big| #3 \big\rangle}
\newcommand{\bra}[1]{\big\langle#1\big|}
\newcommand{\ket}[1]{\big|#1\big\rangle}
\newcommand{\bigket}[1]{\bigl|#1\bigr\rangle}
\newcommand{\textket}[1]{|#1\rangle}
  %double bras and kets
	\newcommand{\dbraket}[2]{\big\langle\big\langle #1 \big| #2 \big\rangle \big\rangle}
  \newcommand{\dketbra}[2]{\big|  #1  \big\rangle\big\rangle \big\langle \big\langle #2 \big| }
  \newcommand{\dbraopket}[3]{\big\langle \big\langle #1 \big| #2 \big| #3 \big\rangle \big\rangle}
  \newcommand{\dket}[1]{\big|#1\big\rangle \big\rangle}
  \newcommand{\dbra}[1]{\big\langle \big\langle#1\big|}
  \newcommand{\dexp}[1]{\big\langle\big\langle #1 \big\rangle \big\rangle}



% Various bracketing commands
\newcommand{\of}[1]{\!\left(#1\right)}
\newcommand{\sqof}[1]{\left[#1\right]}
\newcommand{\cuof}[1]{\left\{#1\right\}}

% commutator and anticommutator
\newcommand{\comm}[2]{\left[#1,#2\right]}
\newcommand{\anticomm}[2]{\left\{#1,#2\right\}}
% sum on nearest neighbor bonds
\newcommand{\bond}{\left\langle i, j \right\rangle}
%\newcommand{\bondsum}{\sum_{\left\langle i, j \right\rangle}}
\newcommand{\nbond}{\left\langle\left\langle i, j \right\rangle\right\rangle}
% 1/2
\newcommand{\half}{\frac{1}{2} }
\newcommand{\thalf}{\tfrac{1}{2} }
% simplifies using the up and down arrows to denote spin
\newcommand{\up}{\uparrow}
\newcommand{\down}{\downarrow}
% Absolute value  
\newcommand{\abs}[1]{\left|#1\right|}

% Roman functions for real and imaginary parts
\newcommand{\re}{\mathrm{Re}}
\newcommand{\im}{\mathrm{Im}}


%Expectation values
\newcommand{\expect}[1]{\left\langle#1\right\rangle}
\newcommand{\pdag}{\phantom{\dagger}}
\newcommand{\pdg}[1]{{#1}^{\phantom{\dagger}}}

\newcommand{\bkap}{\bar{\glide}}
\newcommand{\bchi}{\bar{\chi}}
\newcommand{\baeta}{\bar{\eta}}
\newcommand{\lin}{\notag \\}



\newcommand{\ab}{\alpha\beta}
\newcommand{\deli}{\Delta^{-1}}


\newcommand{\ra}{{R\,\alpha}}
\newcommand{\rax}{{R+\vec{x}\,\alpha}}

\newcommand{\rb}{{R'\,\beta}}
\newcommand{\rarb}{{R\,\alpha};R'\,\beta}
\newcommand{\zth}{\mathbb{Z}_3}


\newcommand{\xin}{x_{\tex{inv}}}
\newcommand{\low}{L$\ddot{\text{o}}$wdin\;}
\newcommand{\tex}[1]{\sma{\text{#1}}}











\newcommand{\kf}{k_{\scriptscriptstyle{F}}}

\newcommand{\bfk}{\boldsymbol{k}}
\newcommand{\bfq}{\boldsymbol{q}}



\newcommand{\bpm}{\begin{pmatrix}}
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\nk}{n_{\boldsymbol{k}'}}
\newcommand{\dk}{\Delta_{\boldsymbol{k}'}}
\newcommand{\Dk}{\Delta_{\boldsymbol{k}}}
\newcommand{\tk}{\tilde{k}}
\newcommand{\tkp}{\tilde{k}'}
\newcommand{\bal}{\begin{align}}
\newcommand{\Ainv}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}

\newcommand{\V}{V_{\text{eff}}}
\newcommand{\si}{\;\text{sin}\,}
\newcommand{\ta}{\;\text{tan}\,}
\newcommand{\co}{\;\text{\text{cos}}\,}
\newcommand{\te}{t_{\text{eff}}}
\newcommand{\ep}{\bar{\epsilon}}



\newcommand{\braa}[1]{\left\langle#1\right|_{\scriptscriptstyle{A}}}
\newcommand{\brab}[1]{\left\langle#1\right|_{\scriptscriptstyle{B}}}

\newcommand{\dg}[1]{#1^{\scriptstyle{\dagger}}}
\newcommand{\bof}[1]{\boldsymbol{#1}}
\newcommand{\sma}[1]{\scriptscriptstyle{#1}}
\newcommand{\po}{{\sma{+}} 1}



\newcommand{\noc}{n_{\sma{{occ}}}}
\newcommand{\ntot}{n_{\sma{{tot}}}}

\newtheorem{definition}{Definition}[section]
